FEVER-OOD: Free Energy Vulnerability Elimination for Robust Out-of-Distribution Detection

Modern machine learning models, that excel on computer vision tasks such as classification and object detection, are often overconfident in their predictions for Out-of-Distribution (OOD) examples, resulting in unpredictable behaviour for open-set environments. Recent works have demonstrated that the free energy score is an effective measure of uncertainty for OOD detection given its close relationship to the data distribution. However, despite free energy-based methods representing a significant empirical advance in OOD detection, our theoretical analysis reveals previously unexplored and inherent vulnerabilities within the free energy score formulation such that in-distribution and OOD instances can have distinct feature representations yet identical free energy scores. This phenomenon occurs when the vector direction representing the feature space difference between the in-distribution and OOD sample lies within the null space of the last layer of a neural-based classifier. To mitigate these issues, we explore lower-dimensional feature spaces to reduce the null space footprint and introduce novel regularisation to maximize the least singular value of the final linear layer, hence enhancing inter-sample free energy separation. We refer to these techniques as Free Energy Vulnerability Elimination for Robust Out-of-Distribution Detection (FEVER-OOD). Our experiments show that FEVER-OOD techniques achieve state of the art OOD detection in Imagenet-100, with average OOD false positive rate (at 95% true positive rate) of 35.83% when used with the baseline Dream-OOD model.

==> tables/cifar10_res_formatted.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{CIFAR-10 Results (ID Acc. $=$ in-distribution accuracy; Null Space Reduction (NSR) methods $=$ our approach).}
\label{table:cifar-10-eval}
\resizebox{0.95\linewidth}{!}{%
\renewcommand{\arraystretch}{1}
\begin{tabular}{llllrrrrrrrrrrrrl}
\hline
\multicolumn{2}{c}{}                                  &                                           &                                         & \multicolumn{12}{c}{OOD Datasets}                                                                                                                                                                                                                                                                                                             &                          \\ \cline{5-16}
\multicolumn{2}{c}{}                                  &                                           &                                         & \multicolumn{2}{l}{Textures}                          & \multicolumn{2}{l}{SHVN}                              & \multicolumn{2}{l}{Places365}                         & \multicolumn{2}{l}{LSUN}                              & \multicolumn{2}{l}{iSUN}                              & \multicolumn{2}{l}{Avg}                               & \multirow{-2}{*}{ID Acc} \\ \cline{5-16}
\multicolumn{2}{c}{\multirow{-3}{*}{Method}}          & \multirow{-3}{*}{$\lambda_\mathit{LSVV}$} & \multirow{-3}{*}{$\lambda_\mathit{CN}$} & \multicolumn{1}{l}{FPR95} & \multicolumn{1}{l}{AUROC} & \multicolumn{1}{l}{FPR95} & \multicolumn{1}{l}{AUROC} & \multicolumn{1}{l}{FPR95} & \multicolumn{1}{l}{AUROC} & \multicolumn{1}{l}{FPR95} & \multicolumn{1}{l}{AUROC} & \multicolumn{1}{l}{FPR95} & \multicolumn{1}{l}{AUROC} & \multicolumn{1}{l}{FPR95} & \multicolumn{1}{l}{AUROC} &                          \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS (baseline)}       &                                           &                                         & 50.62                     & 86.98                     & 42.47                     & 90.53                     & 40.17                     & 89.72                     & 7.94                      & 98.34                     & 25.30                     & 95.28                     & 33.30                     & 92.17                     & 94.85                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS}       & 1.0                                       &                                         & 48.12                     & 88.43                     & 39.59                     & 91.64                     & 34.42                     & 92.15                     & 6.51                      & 98.49                     & 17.14                     & 96.84                     & 29.16                     & 93.51                     & 94.48                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS}       &                                           & 0.1                                     & 47.01                     & 86.15                     & 29.54                     & 93.61                     & 42.00                     & 88.45                     & 7.71                      & 98.31                     & 29.82                     & 94.47                     & 31.22                     & 92.20                     & 94.63                    \\
\multicolumn{2}{l}{VOS-NSR96}                         &                                           &                                         & 50.59                     & 88.79                     & \textbf{25.49}            & \textbf{95.26}            & 39.09                     & 91.90                     & 7.36                      & 98.42                     & 26.90                     & 95.55                     & 29.89                     & 93.98                     & 94.69                    \\
\multicolumn{2}{l}{VOS-NSR96}                         & 1.0                                       &                                         & \textbf{35.21}            & \textbf{93.40}            & 42.84                     & 93.12                     & \textbf{32.66}            & \textbf{93.37}            & \textbf{3.24}             & \textbf{99.26}            & \textbf{13.44}            & \textbf{97.65}            & \textbf{25.48}            & \textbf{95.36}            & 94.84                    \\
\multicolumn{2}{l}{VOS-NSR96}                         &                                           & 0.1                                     & 39.97                     & 91.77                     & 39.80                     & 93.96                     & 39.16                     & 90.69                     & 4.35                      & 99.00                     & 24.23                     & 95.59                     & 29.50                     & 94.20                     & 94.55                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR64} &                                           &                                         & 45.05                     & 89.40                     & 45.37                     & 91.58                     & 36.74                     & 91.53                     & 6.36                      & 98.74                     & 22.48                     & 95.95                     & 31.20                     & 93.44                     & 94.73                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR64} & 1.0                                       &                                         & 44.04                     & 90.53                     & 34.13                     & 95.16                     & 36.39                     & 92.43                     & 5.28                      & 98.74                     & 19.74                     & 96.66                     & 27.92                     & 94.70                     & 94.80                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR64} &                                           & 0.001                                   & 42.12                     & 91.01                     & 43.18                     & 93.20                     & 36.23                     & 91.71                     & 6.66                      & 98.71                     & 25.40                     & 95.01                     & 30.72                     & 93.93                     & 94.75                    \\
\multicolumn{2}{l}{VOS-NSR32}                         &                                           &                                         & 38.39                     & 91.87                     & 66.94                     & 88.35                     & 37.35                     & 91.68                     & 5.73                      & 98.86                     & 29.84                     & 94.58                     & 35.65                     & 93.07                     & 94.64                    \\
\multicolumn{2}{l}{VOS-NSR32}                         & 0.001                                     &                                         & 47.80                     & 89.19                     & 40.57                     & 93.90                     & 38.48                     & 91.78                     & 5.95                      & 98.73                     & 23.04                     & 95.94                     & 31.17                     & 93.91                     & 94.78                    \\
\multicolumn{2}{l}{VOS-NSR32}                         &                                           & 0.1                                     & 43.86                     & 89.65                     & 28.08                     & 95.23                     & 41.33                     & 90.33                     & 5.31                      & 98.94                     & 29.42                     & 94.76                     & 29.60                     & 93.78                     & 95.05                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR10} &                                           &                                         & 54.56                     & 88.86                     & 33.75                     & 94.80                     & 44.43                     & 90.98                     & 10.48                     & 98.25                     & 42.68                     & 92.81                     & 37.18                     & 93.14                     & 89.64                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR10} & 0.01                                      &                                         & 59.37                     & 86.68                     & 35.98                     & 94.36                     & 41.52                     & 89.65                     & 10.48                     & 98.01                     & 32.60                     & 94.25                     & 35.99                     & 92.59                     & 94.34                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR10} &                                           & 0.001                                   & 59.02                     & 86.46                     & 67.06                     & 88.05                     & 52.25                     & 88.07                     & 19.99                     & 96.56                     & 28.31                     & 95.14                     & 45.33                     & 90.86                     & 88.73                    \\ \hline
\multicolumn{2}{l}{FFS  (baseline)}                               &                                           &                                         & 46.01                     & 87.28                     & 48.73                     & 88.09                     & 41.39                     & 89.01                     & 5.96                      & 98.79                     & 27.71                     & 94.67                     & 33.96                     & 91.57                     & 94.65                    \\
\multicolumn{2}{l}{FFS}                               & 0.001                                     &                                         & 43.94                     & 87.39                     & 22.05                     & 94.74                     & 40.12                     & 89.11                     & 3.21                      & 99.29                     & 16.88                     & 96.52                     & 25.24                     & 93.41                     & 95.08                    \\
\multicolumn{2}{l}{FFS}                               &                                           & 1.0                                     & 44.37                     & 88.12                     & 32.82                     & 92.39                     & 43.39                     & 88.35                     & 4.98                      & 98.92                     & \textbf{9.18}             & \textbf{98.11}            & 26.95                     & 93.18                     & 94.74                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}FFS-NSR96} &                                           &                                         & 47.63                     & 88.64                     & 29.13                     & 95.29                     & 38.13                     & 91.64                     & 4.50                      & 99.03                     & 20.40                     & 96.50                     & 27.96                     & 94.22                     & 94.54                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}FFS-NSR96} & 1.0                                       &                                         & 43.00                     & \textbf{91.85}            & 30.14                     & 94.81                     & \textbf{32.81}            & \textbf{93.10}            & 4.09                      & 99.12                     & 14.61                     & 97.43                     & 24.93                     & \textbf{95.26}            & 94.81                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}FFS-NSR96} &                                           & 0.001                                   & 44.37                     & 90.33                     & 28.56                     & 95.37                     & 39.05                     & 91.59                     & 4.59                      & 99.10                     & 24.73                     & 95.47                     & 28.26                     & 94.37                     & 94.83                    \\
\multicolumn{2}{l}{FFS-NSR64}                         &                                           &                                         & 48.24                     & 89.67                     & 45.38                     & 89.67                     & 38.43                     & 90.80                     & 3.99                      & 99.15                     & 33.55                     & 92.91                     & 33.92                     & 92.44                     & 94.77                    \\
\multicolumn{2}{l}{FFS-NSR64}                         & 1.0                                       &                                         & 43.41                     & 90.96                     & 31.30                     & 93.96                     & 36.52                     & 92.07                     & 3.18                      & 99.22                     & 10.23                     & 98.00                     & 24.93                     & 94.84                     & 94.61                    \\
\multicolumn{2}{l}{FFS-NSR64}                         &                                           & 0.001                                   & 44.01                     & 90.36                     & \textbf{16.97}            & \textbf{96.71}            & 42.08                     & 89.65                     & 3.93                      & 99.20                     & 13.80                     & 97.43                     & \textbf{24.16}            & 94.67                     & 94.91                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}FFS-NSR32} &                                           &                                         & 40.88                     & 90.57                     & 38.84                     & 91.25                     & 43.32                     & 89.74                     & 4.13                      & 99.11                     & 26.67                     & 94.77                     & 30.77                     & 93.09                     & 94.57                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}FFS-NSR32} & 0.001                                     &                                         & 45.18                     & 89.44                     & 28.32                     & 95.35                     & 38.69                     & 91.27                     & \textbf{3.01}             & \textbf{99.30}            & 24.83                     & 95.59                     & 28.01                     & 94.19                     & 94.69                    \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}FFS-NSR32} &                                           & 0.01                                    & \textbf{42.26}            & 90.58                     & 33.15                     & 95.00                     & 42.16                     & 90.37                     & 3.91                      & 99.22                     & 21.71                     & 96.36                     & 28.64                     & 94.31                     & 94.82                    \\
\multicolumn{2}{l}{FFS-NSR10}                         &                                           &                                         & 57.67                     & 82.43                     & 46.68                     & 89.41                     & 46.81                     & 87.28                     & 12.56                     & 97.52                     & 28.66                     & 94.62                     & 38.48                     & 90.25                     & 94.72                    \\
\multicolumn{2}{l}{FFS-NSR10}                         & 0.001                                     &                                         & 56.40                     & 86.41                     & 46.42                     & 92.16                     & 39.34                     & 90.55                     & 6.71                      & 98.62                     & 22.77                     & 96.14                     & 34.33                     & 92.78                     & 94.55                    \\
\multicolumn{2}{l}{FFS-NSR10}                         &                                           & 0.001                                   & 55.59                     & 84.27                     & 74.97                     & 80.77                     & 36.36                     & 91.23                     & 9.75                      & 97.99                     & 31.69                     & 93.16                     & 41.67                     & 89.48                     & 94.49                    \\ \hline
\end{tabular}%
}
\renewcommand{\arraystretch}{1}
\end{table*}

==> tables/oln-ssos_det_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{OLN-SSOS results with PASCAL VOC as in-distribution.}
\label{table:olnssos-det-eval}
\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{1}
\begin{tabular}{llllrrrrr}
\hline
\multicolumn{2}{c}{}                                   &                                           &                                         & \multicolumn{4}{c}{OOD Datasets}                                                                              & \multicolumn{1}{l}{}                      \\ \cline{5-8}
\multicolumn{2}{c}{}                                   &                                           &                                         & \multicolumn{2}{l}{MS-COCO}                           & \multicolumn{2}{l}{OpenImages}                        & \multicolumn{1}{l}{}                      \\ \cline{5-8}
\multicolumn{2}{c}{\multirow{-3}{*}{Method}}           & \multirow{-3}{*}{$\lambda_\mathit{LSVV}$} & \multirow{-3}{*}{$\lambda_\mathit{CN}$} & \multicolumn{1}{l}{FPR95} & \multicolumn{1}{l}{AUROC} & \multicolumn{1}{l}{FPR95} & \multicolumn{1}{l}{AUROC} & \multicolumn{1}{l}{\multirow{-3}{*}{mAP}} \\ \cline{1-8}
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS}        &                                           &                                         &                           &                           &                           & \textbf{}                 &                                           \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS}        &                                           &                                         &                           &                           &                           &                           &                                           \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS}        &                                           &                                         &                           &                           &                           &                           &                                           \\
\multicolumn{2}{l}{VOS-NSR768}                         &                                           &                                         &                           &                           &                           &                           &                                           \\
\multicolumn{2}{l}{VOS-NSR768}                         &                                           &                                         &                           &                           &                           &                           &                                           \\
\multicolumn{2}{l}{VOS-NSR768}                         &                                           &                                         & \textbf{}                 &                           & \textbf{}                 &                           &                                           \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR512} &                                           &                                         &                           & \cellcolor[HTML]{EFEFEF}  & \cellcolor[HTML]{EFEFEF}  &                           &                                           \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR512} &                                           &                                         &                           & \cellcolor[HTML]{EFEFEF}  & \cellcolor[HTML]{EFEFEF}  &                           &                                           \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}VOS-NSR512} &                                           &                                         &                           & \cellcolor[HTML]{EFEFEF}  & \cellcolor[HTML]{EFEFEF}  &                           &                                           \\
\multicolumn{2}{l}{VOS-NSR256}                         &                                           &                                         &                           & \textbf{}                 &                           &                           &                                           \\
\multicolumn{2}{l}{VOS-NSR256}                         &                                           &                                         &                           &                           &                           &                           &                                           \\
\multicolumn{2}{l}{VOS-NSR256}                         &                                           &                                         &                           &                           &                           &                           &                                           \\ \hline
\end{tabular}%
}
\renewcommand{\arraystretch}{1}
\end{table}
